Algebraic Property Graphs

We present a case study in applied category theory written from the point of view of an applied domain: the formalization of the widely-used property graphs data model in an enterprise setting using elementary constructions from type theory and category theory, including limit and co-limit sketches. Observing that algebraic data types are a common foundation of most of the enterprise schema languages we deal with in practice, for graph data or otherwise, we introduce a type theory for algebraic property graphs wherein the types denote both algebraic data types in the sense of functional programming and join-union E/R diagrams in the sense of database theory. We also provide theoretical foundations for graph transformation along schema mappings with by-construction guarantees of semantic consistency. Our data model originated as a formalization of a data integration toolkit developed at Uber which carries data and schemas along composable mappings between data interchange languages such as Apache Avro, Apache Thrift, and Protocol Buffers, and graph languages including RDF with OWL or SHACL-based schemas.

==> acknowledgements.tex <==
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
{\bf Acknowledgements.}  
We would particularly like to thank Jan Hidders for his early contributions to this work.
Jeffrey Brown, Marko A. Rodriguez, Gregory Sharp, and Henry Story provided valuable feedback on this paper, while many other individuals in the graph database community, at Uber, and at Conexus AI have motivated and influenced our solution.
David Spivak and Gregory Malecha gave valuable guidance about category theory and Coq, respectively.


==> category-theory.tex <==
\section{Review of Category Theory}
\label{section.ct}

In this section, we review standard definitions and results from category theory~\cite{awodey2010ct}\cite{mac2013categories}\cite{fong2019invitation}, which serves as a meta-mathematics between various mathematical fields.
For example, using category theory we are able to transport theorems from algebra to topology.
As such, it is a natural choice for describing families of related data models, and we are far from alone in proposing its use in this manner; for example, see \cite{Alagic:2001:MTG:648294.754671} and \cite{Fleming:2003:DC:770018.770021}.

%In this section, by a {\it graph} $G$ we mean a set of {\it vertices} $V$, a set of {\it edges} $E$, and source and target functions $s, t : E \to V$ i.e., a directed multi-graph.  
%We make this definition to avoid writing ``directed, multi-'' in front of ``graph'' in many places.  

\subsection{Categories}

% \subsubsection{Alternate #1}

% A {\it category} $\mathcal{C}$ consists of a set, ${\sf Ob}(\mathcal{C})$, the elements of which we call {\it objects}; a set ${\sf Mor}(\mathcal{C})$, the elements of which we call {\it morphisms}; functions ${\sf dom_\mathcal{C},cod_\mathcal{C}} : {\sf Mor}(\mathcal{C}) \to {\sf Ob}(\mathcal{C})$ called {\it domain} and {\it co-domain}; a function ${\sf id}_\mathcal{C} : {\sf Ob}(\mathcal{C}) \to {\sf Mor}(\mathcal{C})$; and a partial function $ \circ_\mathcal{C} : {\sf Mor}(\mathcal{C}) \times {\sf Mor}(\mathcal{C}) \to {\sf Mor}(\mathcal{C})$ called {\it composition} such that (where we omit the sub-scripted $\mathcal{C}$):
% $$
% {\sf dom}({\sf id}(o)) \ = \ {\sf cod}({\sf id}(o)) \ = \ o
% $$
% $$
% {\sf cod}(g) = {\sf dom}(f) \ \Rightarrow \ {\sf dom}(f \circ g) = {\sf dom}(g) 
% $$
% $$
% {\sf cod}(g) = {\sf dom}(f) \ \Rightarrow \ {\sf  \sf cod}(f \circ g) = {\sf cod}(f)
% $$
% $$
% {\sf id}({\sf dom}(f)) \circ f \ = \ f \ =  \ {\sf id}({\sf cod}(f)) \circ f
% $$
% $$
% ( \ {\sf cod}(g) = {\sf dom}(f) \wedge {\sf cod}(h) = {\sf dom}(g) \Rightarrow
% $$
% $$
% (f \circ g) \circ h = f \circ (g \circ h) \ )
% $$

% \subsubsection{Alternate #2}

A {\it category} $C$ is an axiomatically-defined algebraic structure similar to a group, ring, or monoid.
Following \cite{awodey2010ct}, a category consists of {\it objects} $A$, $B$, $C$, ... and {\it arrows} (also called {\it morphisms}) $f$, $g$, $h$, ... such that: 
\begin{itemize}
    \item For every arrow $f$ there is an object $cod(f)$ called the {\it codomain} of $f$ and an object $dom(f)$ called the {\it domain} of $f$. If $c_1 = cod(f)$ and $c_2 = dom(f)$, we may write $f : c_1 \rightarrow c_2$. Visually: 
    $$
    \xymatrix{
    c_1 \ar[rr]^f & & c_2
    }
    $$
    \item For every arrow $f : c_1 \rightarrow c_2$ and arrow $g : c_2 \rightarrow c_3$ there is an arrow $g \circ f : c_1 \rightarrow c_3$ called the {\it composite} of $f$ and $g$:
    $$
    \xymatrix{
     c_1 \ar[rr]^f \ar@/_1pc/[rrrr]_{g \circ f} & & c_2 \ar[rr]^g && c_3
    }
    $$
    \item Composition is {\it associative}, i.e. $h \circ (g \circ f) = (h \circ g) \circ f$ for arbitrary $f$, $g$, and $h$.
    \item For every object $c$ there is an {\it identity arrow} ${\sf id}_c : c \rightarrow c$:
    $$
    \xymatrix{
    c \ar@(r,u)[]_{{\sf id}_c} 
    }
    $$
    \item Furthermore, for any $f : c_1 \rightarrow c_2$, $f \circ {\sf id}_{c_1} = f = {\sf id}_{c_2} \circ f$.
\end{itemize}
% \subsubsection{Original}
%   It consists of:
% \begin{itemize}
% \item a set, ${\sf Ob}(C)$, the members of which we call {\it objects}, and
% \item for every two objects $c_1, c_2$, a set $C(c_1, c_2)$, the members of which we call {\it morphisms} (or {\it arrows}) from $c_1$ to $c_2$, and
% \item for every three objects $c_1,c_2,c_3$, a function $\circ_{c_1,c_2,c_3} : $ $C(c_2,c_3) $ $\times$ $ C(c_1,c_2) \to C(c_1,c_3)$, which we call {\it composition}, and
% \item for every object $c$, a dinstiguished arrow ${\sf id}_c \in C(c,c)$, which we call the {\it identity} for $c$. 
% \end{itemize}
% We may write $f : c_1 \to c_2$ instead of $f \in C(c_1,c_2)$, and drop object subscripts on ${\sf id}$ and $\circ$, when doing so does not create ambiguity.  
% The data above must obey axioms stating that $\circ$ is associative and ${\sf id}$ is its unit:
% $$
% {\sf id} \circ f = f \ \ \ \ f \circ {\sf id} = f \ \ \ \ f \circ (g \circ h) = (f \circ g) \circ h
% $$
An example category with three objects and six arrows is shown below.
$$
\xymatrix{
c_1 \ar@(l,u)[]^{{\sf id}_{c_1}} \ar[rr]^f \ar@/_1pc/[rrrr]_{g \circ f} & & c_2 \ar[rr]^g \ar@(l,u)[]^{{\sf id}_{c_2}} &&  c_3 \ar@(l,u)[]^{{\sf id}_{c_3}} \\
%F(c_1) \ar[r]_{F(f)}& F(c_2) \\ 
}
$$

In the following, the objects of a category $C$ will be denoted ${\sf Ob}(C)$, and the set of all arrows from object $c_1$ to object $c_2$ in $C$ will be denoted $C(c_1, c_2)$.
Two arrows $f : c_1 \to c_2$ and $g : c_2 \to c_1$ such that $f \circ g = {\sf id}$ and $g \circ f = {\sf id}$ are said to be an {\it isomorphism}. 

Every category corresponds to a labeled graph, its objects being vertices, and its arrows being edges.
Many categories may correspond to the same graph.
Conversely, to every graph $G$ there is a category, the so-called {\it free category} generated by $G$ has for objects the vertices of $G$, and for arrows $v_1 \to v_2$ the (possibly 0-length) paths from $v_1$ to $v_2$ in $G$.
A graph inducing the category example from above is:
$$
\xymatrix{
c_1  \ar[rr]^f & & c_2 \ar[rr]^g  & & c_3 
% F(c_1) \ar[r]_{F(f)}& F(c_2) \\ 
}
$$  
% As another example, the graph with two vertices $v_1, v_2$ and two edges $f : v_1 \to v_2$ and $g : v_2 \to v_1$ gives rise to a category with two objects, $v_1, v_2$ and infinitely many morphisms in the guise of all paths through $g$, namely, $[]:v_1\to v_1, [f]:v_1 \to v_2, [f,g] : v_1 \to v_1$, etc. 

\subsection{Functors}

A {\it functor} $F : C \to D$ between categories $C$ and $D$ consists of:
\begin{itemize}
    \item  a function $F : {\sf Ob}(C) \to {\sf Ob}(D)$, and
    \item for every $c_1,c_2 \in {\sf Ob}(C)$, a function $F_{c_1,c_2} : C(c_1,c_2) \to D(F(c_1),F(c_2))$, where we may omit object subscripts when they can be inferred from context, such that 
\end{itemize}
$$
F({\sf id}_c) = {\sf id}_{F(c)} \ \ \ \ \ \ F(f \circ g) = F(f) \circ F(g).
$$
The image of the example category above under a functor $F$ is:
$$
\xymatrix{
 F(c_1) \ar@(l,u)[]^{{\sf id}_{F(c_1)}} \ar[rr]^{F(f)} \ar@/_1pc/[rrrr]_{F(g) \circ F(f)} & & F(c_2) \ar[rr]^{F(g)} \ar@(l,u)[]^{{\sf id}_{F(c_2)}} && F(c_3) \ar@(l,u)[]^{{\sf id}_{F(c_3)}}  \\
}
$$
\subsection{Natural Transformations}
A {\it natural transformation} $h : F \to G$ between functors $F, G : C \to D$ consists of a set of morphisms (arrows) $h_c : F(c) \to G(c)$, indexed by objects in $C$, called the {\it components} of $h$,
 such that for every $f : c_1 \to c_2$ in $C$, 
$
h_{c_2} \circ F(f) = G(f) \circ h_{c_1}
$.
This set of equations may be conveniently rendered as a {\it commutative diagram}: 
$$
\xymatrix{
F(c_1) \ar[d]_{h_{c_1}} \ar[r]^{F(f)} & F(c_2) \ar[d]^{h_{c_2}} \\
G(c_1) \ar[r]_{G(f)}& G(c_2) \\ 
}
$$
The diagram above consists of a {\it square} (the four morphisms) indicating that all paths that start at the same node and end at the same node are to {\it commute} (be equal) in $D$; in this case, there are two such paths.  The upper-left two morphims $ \cdot \leftarrow \cdot \to \cdot$ of a square are called a {\it span}, and the bottom-right two morphisms $\cdot \to \cdot \leftarrow \cdot$ are called a {\it co-span}.  
%Given a set of commutative squares (equivalently, {\it equations}) $E$ in category $C$, we can form the {\it quotient} category $C/E$, whose morphisms are equivalence classes of morphisms in $C$ modulo the squares in $E$.

A natural transformation is called a {\it natural isomorphism} when all of its components are isomorphisms. 

\subsection{Universal Constructions}
\label{sec:universal-constructions}

A {\it terminal} object $1$ in a category is such that for every object $c$, there is a unique morphism $\top_c : c \to 1$ (read ``top'').
Dually, an {\it initial} object $0$ is such that for every object $c$, there is a unique morphism $\bot_c : 0 \to c$ (read ``bottom'').
Like all constructions described by {\it universal properties}, terminal and initial objects are unique up to unique isomorphism, provided they exist.
Such objects may be familiar to users of functional programming languages; e.g., $\texttt{()}$ and $\texttt{Void}$ are the terminal and initial objects, respectively, of the category ${\sf Hask}$ of idealized Haskell programs.

For objects $A$ and $B$ in a category, a {\it product} of $A$ and $B$ is an object $A \times B$, morphisms ${\sf fst} : A \times B \to A$ and ${\sf snd} : A \times B \to B$ called {\it projections}, such that for all morphisms $f : C \to A$ and $g : C \to B$ there is a unique morphism $(f, g) : C \to A \times B$ called the {\it pairing} of $f$ and $g$ making the left diagram below commute.
%For example, the basic product type in Haskell is an ordered pair \texttt{(a, b)} for which \texttt{fst} produces objects of type \texttt{a} and \texttt{snd} produces objects of type \texttt{b}.

Dually, a {\it co-product} of $A$ and $B$ is an object $A + B$, morphisms ${\sf inl} : A \to A + B$ and ${\sf inr} : B \to A + B$ called {\it injections}, such that for all morphisms $f: A \to C$ and $g : B \to C$, there is a unique morphism $(f \ | \ g) : A + B \to C$ called the {\it case analysis} of $f$ and $g$ making the diagram below on the right commute.
%For example, the basic coproduct type in Haskell is \texttt{Either a b}; one constructs the ${\sf inl}$ or ``left'' variant by applying the function \texttt{Left} to an object of type \texttt{a}, and the ${\sf inr}$ or ``right'' variant by applying the function \texttt{Right} to an object of type \texttt{b}.
$$
\xymatrix{
 & C \ar@{-->}[d]_{(f, g)} \ar[dl]_{f} \ar[dr]^{g} & \\
A & \ar[l]^{{\sf fst}} \ar[r]_{{\sf snd}} A \times B & B \\ 
} \ \ \ \ \ \ \ \ \ \ \ 
\xymatrix{
 & C  & \\
A \ar[r]_{{\sf inl}}  \ar[ur]^{f}  &   A + B \ar@{-->}[u]^{(f | g)} & \ar[l]^{{\sf inr}} B  \ar[ul]_{g} \\ 
}
$$
Given $f : A \to C$ and $g : B \to D$, we define: 
$$f \times g : A \times B \to C \times D \ := \  (f \circ {\sf fst} \ , \ g \circ {\sf snd})
$$
$$
f + g : A + B \to C + D \ := ({\sf inl}  \circ f \ | \ {\sf inr} \circ g)$$  
A category that has (co-)products is called {\it (co-)cartesian} and a functor that preserves (co-)products (i.e., if $X$ is a (co-)product, so is $F(X)$) is also called {\it (co-)cartesian}.  
Because terminal and initial objects are identity objects for products and co-products, they serve as the degenerate, 0-ary versions of products and co-products and are included when we require that a category ``have products/co-products''. 

%To {\it pull back} a co-span $C \to_k D \leftarrow_g B$ as below is to construct object $A$, sometimes written $C \times^{k,g}_D B$, and morphisms $C \leftarrow_{h} A \to_f B$ such that $g \circ f = k \circ h$, and moreover, such that for any other such $A', h', f'$ where $g \circ f' = k \circ h'$, there is a unique morphism $m : A' \to A$ making $f' = f \circ m$ and $h' = h \circ m$.  
%To {\it push out} a span $C \leftarrow_h A \to_f B$ as below is to construct object $D$,  sometimes written $C +_A^{h,f} B$, and morphisms $C \to_k D \leftarrow_g B$ such that $g \circ f = k \circ h$ from $C \leftarrow_h A \to_f B$, such that for any other such $D', k', g'$ where $g' \circ f = k' \circ h$, there is a unique morphism $m : D \to D'$ making $k' = m \circ k$ and $g' = m \circ g$.

%$$
%\xymatrix{
%A' \ar@/^/[rrd]^{f'} \ar@/_/[rdd]_{h'} \ar@{.>}[rd]^m & %\\
%& A \ar[d]_{h} \ar[r]^f & B \ar[d]^{g} \\
%& C \ar[r]_{k} & D \\ 
%}
%\ \ \ \ \ \ \ \ \ \ \ \ \ \ 
%\xymatrix{
% A \ar[d]_{h} \ar[r]^f & B \ar[d]^{g} \ar@/^/[rdd]_{g'} %& \\
% C \ar[r]_{k} \ar@/_/[rrd]^{k'} & D \ar@{.>}[rd]^m & \\
% & & D'   & \\
%}
%$$
%A pullback with terminal $D$ is a product, and a pushout %with initial $A$ is a co-product.  A category with all pullbacks and a terminal object is said to have all {\it limits}; dually, having all pushouts and an initial object means having all {\it co-limits}.  

%The {\it equalizer} of two morphisms $f : B \to C$ and $g : B \to C$ is an object ${\sf Eq}(f,g)$ and morphism ${\sf eq} : {\sf Eq}(f,g) \to B$ such that $f \circ {\sf eq}  = g \circ {\sf eq}$, and moreover, for any $A$ and $m : A \to B$ such that $f \circ m = g \circ m$, there is a unique $u : A \to {\sf Eq}(f,g)$ such that $m = {\sf eq} \circ u$.  Dually, the {\it co-equalizer} of two morphisms $f : B \to C$ and $g : B \to C$ is an object ${\sf CoEq}(f,g)$ and morphism ${\sf coeq} : B \to {\sf Eq}(f,g)$ such that ${\sf coeq} \circ f = {\sf coeq} \circ g$, and moreover, for any $A$ and $m : C \to A$ such that $m \circ f = m \circ g$, there is a unique $u : {\sf CoEq}(f,g) \to A$ such that $m = u \circ {\sf coeq}$:
%$$
%\xymatrix{
%{\sf Eq}(f,g) \ar[r]^{\sf eq} & B \ar@/^/[r]^f \ar@/_/[r]_g & C \\
%A \ar[ru]_m \ar@{-->}[u]^u
%} \ \ \ \ \ \ \ 
%\xymatrix{
% B \ar@/^/[r]^f \ar@/_/[r]_g  & C \ar[dr]_m  \ar[r]^{\sf %coeq \ \ } & {\sf CoEq}(f,g) \ar@{-->}[d]^u  \\
%& & A  
%}
%$$

%A pullback is equivalent to a product followed by an equalizer, and vice-versa.  A pushout is equivalent to a co-product followed by a co-equalizer, and vice versa.  Hence we will freely interchange various kinds of limits and co-limits in this paper.  

\subsection{Examples}
\begin{itemize}
\item The category of sets and total functions,  ${\sf Set}$, has for objects all the ``small'' sets in some set theory, such as Zermelo-Fraenkel set theory, and a morphism $X$ to  $Y$ is a total function $X \to Y$ represented as a set.
The initial object is the empty set and every singleton set is terminal.
Products are cartesian products, and co-products are disjoint unions.  

%The equalizer of two morphisms $f,g : B \to C$ is the set $ \{ b \in B \ | \ f(b) = g(b) \}$ and inclusion function, and the co-equalizer of $f,g$ is the set of equivalence classes of $C$ under the equivalence relation $\cong$ induced by $f(b) \cong g(b)$ for every $b \in B$, along with the function taking each element of $C$ to its equivalence class.
%The pullback of a co-span of morphisms $C \to_k D \leftarrow_g B$ is the set of pairs $(c,b)$ such that $k(c) = g(b)$ for every $c \in C$ and $b \in B$ (i.e. a join).  
%The pushout of a span of morphisms $C \leftarrow_{h} A \to_f B$ is the disjoint union of $C$ and $B$ modulo the equivalence relation generated by $h(a) = f(a)$ for every $a \in A$ (a kind of recursive tuple-merge of the disjoint union). 

\item  The category ${\sf Rel}$ has ``small'' sets for objects and binary relations as morphisms.  Products and co-products coincide in ${\sf Rel}$ (it is {\it self-dual}) and both are given by disjoint union.  
%Pullbacks and pushouts are rare.

\item Programming languages often form categories, with types $t$ as objects programs taking inputs of type $t_1$ and returning outputs of type $t_2$ as morphisms $t_1 \to t_2$.  Products and co-products are common.  

%, but equalizers and co-equalizers are not, perhaps because they correspond to dependent types (since they are objects depending on morphisms).

%\item In the category of rings (with identity) {\sf Ring} the product corresponds to the ``direct'' product of rings, and the co-product to the ``free'' product of rings.  The terminal ring has a single element corresponding to both the additive and multiplicative identity, and the initial ring is the ring of integers.  The equalizer in {\sf Ring} is just the set-theoretic equalizer (the equalizer of two ring homomorphisms is always a subring).
%The co-equalizer of two ring homomorphisms $f$ and $g$ from $R$ to $S$ is the quotient of $S$ by the ideal generated by all elements of the form $f(r) - g(r)$ for $r \in R$.

\end{itemize}


==> defunct.tex <==

\subsection{Conjunctive APG Queries}

APGs support generalizations of most operations from set theory and relational algebra (RA).  To make this statement precise, we arrange APGs into a category {\sf APG} and prove the existence of:

\begin{itemize}
    \item initial objects in {\sf APG}, which correspond to the empty set in the category of sets, {\sf Set}, and the empty table (of some given arity) in RA; and
    \item terminal objects in {\sf APG}, which correspond to singleton (one element) sets in {\sf Set} and singleton tables (of some given arity) in RA; and
    \item product objects in {\sf APG}, which correspond to the cartesian product in {\sf Set} and {\tt CROSS JOIN} in RA; and
    \item co-product objects in {\sf APG}, which correspond to disjoint union in {\sf Set} and (roughly) {\tt OUTER UNION ALL} in RA; and
    \item equalizer objects in {\sf APG}, which corresponds to a bounded comprehension principle in {\sf Set} and {\tt SELECT * FROM $X$ AS $x$ WHERE $p(x)$} in RA.
\end{itemize}

Our choice of above universal constructions (product, equalizer, etc.) is canonical and motivated by a desire to interpret the syntax of unions of conjunctive queries, 0-ary records, and other constructions that occur in graph processing in practice.  In other words, product objects and projection morphisms in a category are exactly the structure required to interpret (possibly 0-ary) tuples/records; equalizer objects and the corresponding filtering morphism is exactly the structure required to interpret the WHERE clause of a query, and so forth~\cite{sketches}.  Hence, the operations of this section can be used directly to answer unions of conjunctive queries on APGs.  It is possible to consider non-monotone operations such as set-difference in the context of APGs using the techniques from algebraic databases~\cite{schultz_wisnesky_2017}, but we leave that for future work.

We begin by defining a {\it morphism of APGs} $h : G_1 \to G_2$ to consists of a function $h_{\pgL} : G_1(\pgL) \to G_2(\pgL)$, and a function $h_{\pgE} : G_1(\pgE) \to G_2(\pgE)$, such that $$h_{\pgL} \circ G_1(\pglambda) = G_2(\pglambda) \circ h_{\pgE}.$$
    We say that $h$ is {\it natural} in $\pglambda$. 

\begin{theorem}
APGs and their morphisms form a bi-cartesian category (category with binary products, binary co-products, initial object, and terminal object) with equalizers, which we call {\sf APG}. 
\end{theorem}
\begin{proof}
Done in Coq.  The identity APG morphism is given by identity functions in {\sf Set}, and APG morphism composition is given by function compositions in {\sf Set}.      We define $0(\pgL) := 0(\pgE) := \pgzero$, and $0(\pglambda) := 0(\pgsigma) := 0(\pgupsilon) := \bot$, as well as $\bot_G : \pgzero \to G$ as the unique pair of functions $(\bot, \bot)$ in {\sf Set}. We define $1(\pgL) := 1(\pgE) := \pgone$, and $1(\pglambda) := 1(\pgsigma) := 1(\pgupsilon) := \ \pgunit$, as well as  $\bot_G : G \to \pgone$ as the unique pair of functions $(\pgunit, \pgunit)$ in {\sf Set}. 

    We define the co-product APG $G_1 + G_2$ as:
      \begin{align*}
      & (G_1 + G_2)(\pgL) \ := \ G_1(\pgL) + G_2(\pgL) \\
      & (G_1 + G_2)(\pgE) \ := \ G_1(\pgE) + G_2(\pgE) \\
      & (G_1 + G_2)(\pglambda) \ := \  G_1(\pglambda) + G_2(\pglambda) \\
      & (G_1 + G_2)(\pgsigma) \ :=    \ \diamond_{\sf inl} G_1(\pgsigma) \ + \ \diamond_{\sf inr} G_2(\pgsigma) \\
      & (G_1 + G_2)(\pgupsilon)\ \ := \ \diamond^{\sf inl}_{\sf inl} G_1(\pgupsilon) \ + \  \diamond^{\sf inr}_{\sf inr} G_2(\pgupsilon)
      \end{align*}
with evident injection APG morphisms $G_1 \to G_1 + G_2$ and $G_2 \to G_1 + G_2$ and case-analysis morphism $(p, q) : G_1 + G_2 \to G$ for every $p : G_1 \to G$ and $q : G_2 \to G$. 
    
    We define the product APG $G_1 \times G_2$ as: 
    \begin{align*}
    (G_1 \times G_2)(\pgL) &:= G_1(\pgL) \times G_2(\pgL) \\
    (G_1 \times G_2)(\pgE) &:= G_1(\pgE) \times G_2(\pgE) \\
    (G_1 \times G_2)(\pglambda) &:= G_1(\pglambda) \times G_2(\pglambda) \\
    (G_1 \times G_2)(\pgsigma)((\pglabel{l_1}, \pglabel{l_2})) \ &:=    \diamond_{(-, l_2)} G_1(\pgsigma)(\pglabel{l_1}) \ \times \ \diamond_{(\pglabel{l_1}, \pglabel{-})} G_2(\pgsigma)(\pglabel{l_2}) \\
    G_1 \times G_2)(\pgupsilon)((\pgelement{e_1}, \pgelement{e_2})) \ &:= 
     \end{align*}
    $$\bigl(\diamond^{(\pgelement{-}, \pgelement{e_2})}_{(\pglabel{-}, G_2(\pglambda)(\pgelement{e_2}))} G_1(\pgupsilon)(\pglabel{e_1}) \ , 
    \diamond^{(\pgelement{e_1}, \pgelement{-})}_{(G_1(\pglambda)(\pgelement{e_1}), \pglabel{-})} G_2(\pgupsilon)(\pgelement{e_2}) \bigr) 
   $$
    with evident projection APG morphisms $G_1 \times G_2 \to G_1$ and $G_1 \times G_2 \to G_2$ and pairing morphism $(p, q) : G \to G_1 \times G_2$ for every $p : G \to G_1$ and $q : G \to G_2$.  
     \item We define the equalizer APG ${\sf Eq}$ for  $h , k : G \to G'$ as
     $$
     {\sf Eq}(\pgL) := \{ \ \pglabel{l} \ | \ h_{\pgL}(\pglabel{l}) = k_{\pgL}(\pglabel{l}), \ \pglabel{l} \in G(\pgL) \  \} 
     $$ $$
     {\sf Eq}(\pgE) := \{ \ \pgelement{e} \ | \ h_{\pgE}(\pgelement{e}) = k_{\pgE}(\pgelement{e}), \ \pgelement{e} \in G(\pgE) \ \}
     $$
     $$
     {\sf Eq}(\pglambda) := G(\pglambda)
     $$
     $$
     {\sf Eq}(\pgsigma)(\pglabel{l}) :=
      \diamond_{\pglabel{l'} \ \mapsto \ {\sf if} \ h_{\pgL}(\pglabel{l'}) = k_{\pgL}(\pglabel{l'}) \ {\sf then} \  \pgone + l' \ {\sf else} \ \pgone }  G(\pgsigma)(\pglabel{l})
     $$
     $$
     {\sf Eq}(\pgupsilon)(\pgelement{e'}) \ :=
     \  \diamond^{\pgelement{e} \ \mapsto \ top}_{\pglabel{l'} \ \mapsto \ bot}   \  G(\pgupsilon)(\pgelement{e'})
     $$
     with
     \begin{align*}
     top \ &:= \ {\sf if} \ h_{\pgL}(G(\lambda)(\pgelement{e})) = k_{\pgL}(G(\lambda)(\pgelement{e})) \ {\sf then} 
     \ top' \ {\sf else} \ \pgunit \\
top' \ &:= \ {\sf if} \ h_{\pgE}(\pgelement{e}) = k_{\pgE}(\pgelement{e}) \ {\sf then} \  {\sf inr}(\pgelement{e}) \ {\sf else} \ {\sf inl}(\pgunit) \\
     bot \ &:= \ {\sf if} \ h_{\pgL}(\pglabel{l'}) = h_{\pgL}(\pglabel{l'}) \ {\sf then} \ \pgone + \pglabel{l'} \ {\sf else} \ \pgone 
     \end{align*}
 and the morphism ${\sf eq} : {\sf Eq} \to G$ easily seen to be an inclusion.  Given a $Q$ and $q : Q \to G$ such that $q \circ h = q \circ k$, we construct $u : Q \to {\sf Eq}$ using similar logic as above.
\end{proof}

%Note also that it is certainly possible to design query languages that do not contain the above operations; for example, relational algebra does not contain a terminal object, in the sense that there is no single relational algebra expression $R$ with the property that $\forall X. R \ \texttt{CROSSJOIN} \ X = X$, even though any singleton set is a solution for $R$; this failure occurs because the notion of empty tuple is technically not domain independent in the sense of Codd~\cite{Doan:2012:PDI:2401764}, precluding e.g. empty select statements in SQL.

\subsection{Merging APGs}
\label{sec.linkage}

Although the category {\sf APG} described in the previous section supports joining APGs relative to an overlap, it does not always support the dual operation, APG merge / pushout (co-product followed by co-equalizer ) relative to an overlap, because the category {\sf APG} does not always admit co-equalizers; for example, co-equalizing APG morphisms $h,j : G \to G'$ such that $G'(\pgL)(h_{\pgL}(\pglabel{l})) = \pgtypelit{Nat}$ and $G'(\pgL)(j_{\pgL}(\pglabel{l})) = \pgtypelit{String}$ is not possible.  So, we move to a different category to obtain co-equalizers: 

\begin{theorem}
For each schema $S$, the APGs on $S$ and the $\pgsigma$-preserving APG morphisms form a category, $S$-{\sf APG}-{\sf Int}.  It has co-equalizers of morphisms $h , j : G \to G'$ when, for $\pgelement{e_1},\pgelement{e_2}\in G'(\pgE)$, $\pgelement{e_1} \sim \pgelement{e_2}$ implies $ G'(\pglambda)(\pgelement{e_1}) = G'(\pglambda)(\pgelement{e_2})$, where $\sim$ is the equivalence relation induced by $h_{\pgE}(\pgelement{e}) \sim j_{\pgE}(\pgelement{e})$ for $\pgelement{e}\in G(\pgE)$.
\end{theorem}
\begin{proof}
Done in Coq.  Our definition of co-equalizer is as follows. 
Let $G$ and $G'$ be APGs such that $G(\pgL) = G'(\pgL)$ and $G(\pgsigma) = G'(\pgsigma)$, and $h , j : G \to G'$ be APG morphisms such that $h_{\pgL} = j_{\pgL} = {\sf id}$ and $\pgelement{e_1} \sim \pgelement{e_2} \Rightarrow G'(\pglambda)(\pgelement{e_1}) = G'(\pglambda)(\pgelement{e_2})$, where $\sim$ is the equivalence relation induced by $h_{\pgE}(\pgelement{e}) \sim j_{\pgE}(\pgelement{e})$ for $\pgelement{e}\in G(\pgE)$.  Writing $G'(\pgE) / \sim$ to indicate the quotient of the set $G'(\pgE)$ by $\sim$ and $[] \ : \ G'(\pgE) \to G'(\pgE) / \sim$ and $[]^{-1}  \ : \ G'(\pgE) / \sim \ \to G'(\pgE)$ as the canonical operations of injecting into an equivalence class and finding a representative for an equivalence class, we define the co-equalizer APG ${\sf CoEq}(h,j)$ as
\begin{align*}
{\sf CoEq}(h,j)(\pgL) = G'(\pgL) \ \ \ 
&{\sf CoEq}(h,j)(\pgsigma) = G'(\pgsigma) \\
{\sf CoEq}(h,j)(\pgE) &= G'(\pgE) / \sim \\
{\sf CoEq}(h,j)(\pglambda) &= G'(\pglambda) \circ []^{-1} \\
{\sf CoEq}(h,j)(\pgupsilon) &= \diamond_{\sf id}^{[]} \circ G'(\pgupsilon) \circ []^{-1}
\end{align*}
with the morphism ${\sf coeq} : G' \to {\sf Coeq}(f,g)$ given by
\begin{align*}
{\sf coeq}_{\pgL} = {\sf id} \ \ \ 
{\sf coeq}_{\pgE} = []
\end{align*}
The mediating morphism of the universal property is also trivial, involving $[]^{-1}$ instead.
\end{proof}
In practice, we expect that most morphisms to be co-equalized will be generated by {\it entity resolution} or {\it record linkage}~\cite{Doan:2012:PDI:2401764} algorithms; when elements are matched based on equality, we obtain the analog of set-theoretic union for APGs.
Note, however, that matching APG elements based on equality can be too fine a notion of  equivalence in situations where element ids are meaningless identifiers, in the sense that for sets, $Y \cong Y'$ (where $\cong$ indicates isomorphism) does not imply either $X \cup Y \cong X \cup Y'$ or $X \cap Y \cong X \cap Y'$.
Methods for obtaining suitable (course-enough) matches are described in~\cite{schultz_wisnesky_2017} and~\cite{wadt}, and their further study in the context of APG is left for future work.

We conclude this section with an example of a simple coarse-enough matching strategy, which is to match two APGs with the same schema, where we require that every element have a primary key that does not contain labels.
We match elements based on equality of those keys.
%In such a circumstance, there is at most one (mono) morphism between APGs~\cite{sketches}. note by ryan: we can't use sketches with this notion of morphism. this may not be a theorem anymore
For example, let $G_1$ and $G_2$ be APGs with one label, $\pglabellit{PlateNumber}$, such that

\begin{footnotesize}
\begin{align*}
G_1(\pgsigma)(\pglabellit{PlateNumber}) & = G_2(\pgsigma)(\pglabellit{PlateNumber}) \\
& = \pgtypelit{String} \times \pgtypelit{String} \times \pgtypelit{String}
\end{align*}
\end{footnotesize}
where the first component is a country id, the second a region id, and the third a regional license plate number:  
\begin{footnotesize}
\begin{align*}
& G_1(\pgE) = \{ \pgelement{p_1}, \pgelement{p_2} \} \ \ \
  G_2(\pgE) = \{ \pgelement{q_1}, \pgelement{q_2} \} \\
& G_1(\pgupsilon)(\pgelement{p_1}) = (\pgvaluelit{"US"}, \pgvaluelit{"CA"}, \pgvaluelit{"6TRJ244"}) \\
& G_1(\pgupsilon)(\pgelement{p_2}) = (\pgvaluelit{"MX"}, \pgvaluelit{"BC"}, \pgvaluelit{"AHD-41-02"}) \\
& G_2(\pgupsilon)(\pgelement{q_1}) = (\pgvaluelit{"US"}, \pgvaluelit{"CA"}, \pgvaluelit{"6TRJ244"}) \\ 
& G_2(\pgupsilon)(\pgelement{q_2}) = (\pgvaluelit{"MX"}, \pgvaluelit{"SON"}, \pgvaluelit{"VUK-17-75"}) 
\end{align*}
\end{footnotesize}

By examining the primary keys, we obtain a matched APG $G$ on the same schema:
\begin{footnotesize}
\begin{align*}
G(\pgE) = \{ (\pgelement{p_1}, \pgelement{q_1}) \} \ \ \ 
G(\pgupsilon)((\pgelement{p_1}, \pgelement{q_1})) = (\pgvaluelit{"US"}, \pgvaluelit{"CA"}, \pgvaluelit{"6TRJ244"})
\end{align*}
\end{footnotesize}
along with inclusion morphisms $G_1 \leftarrow G \to G_2$ ; hence we have constructed a span of APGs.  If we go on to pushout this span, we obtained the merged APG $G_1 +_G G_2:$

\begin{footnotesize}
\begin{align*}
& (G_1 +_G G_2)(\pgE) = \{ (\pgelement{p_1}, \pgelement{q_1}), \pgelement{p_2} , \pgelement{q_2} \} \\
& (G_1 +_G  G_2)(\pgupsilon)((\pgelement{p_1}, \pgelement{q_1})) = (\pgvaluelit{"US"}, \pgvaluelit{"CA"}, \pgvaluelit{"6TRJ244"}) \\
& (G_1 +_G  G_2)(\pgupsilon)(\pgelement{p_2}) = (\pgvaluelit{"MX"}, \pgvaluelit{"BC"}, \pgvaluelit{"AHD-41-02"}) \\
& (G_1 +_G  G_2)(\pgupsilon)(\pgelement{q_2}) = (\pgvaluelit{"MX"}, \pgvaluelit{"SON"}, \pgvaluelit{"VUK-17-75"}) 
\end{align*}
\end{footnotesize}
In this way, we can easily compose two such graphs into a larger graph, an operation which has proven to be extremely useful in the context of RDF triple stores, but which tends to be ill-defined and difficult in the context of property graphs.
The approach works just as well with typical, simple vertex and edge ids as it does with the compound keys in the above example.  Note also that although this example finds a co-span and computes a pushout, it can easily be re-phrased to find a pair of parallel morphisms and compute a co-equalizer~\cite{awodey2010ct}.

==> extras/extensions.tex <==
\section{Appendix Indexed Algebraic Datatypes}
\label{section.adts_extension}

In this section we define the free (indexed) bi-cartesian category $\mathcal{A}_B$ over a category $B$,  following the presentation of~\cite{seely}. A {\it type} is a term in the grammar:
$$
t\ ::=  \ b \ \ (b \in {\sf Ob}(B)) \ \ | \ \ $$ $$ \ \ \ \ \times_{i \in l}. t_i \ \ (l \in {\sf Ob}({\sf Set})) \ \ \ \ | \ \ \ \ +_{i \in l}. t_i \ \ (l \in {\sf Ob}({\sf Set}))
$$
A morphism is an equivalence class of terms in the grammar:
$$
e : t_1 \to t_2 \ ::= \
(e_2 : t_2 \to t_3 \ \circ \ e_1 : t_1 \to t_2) \  : \ t_1 \to t_3 
$$
$$
b_{t_1,t_2} \ : \ p_1 \to p_2 \ \ (b \in B(p_1, p_2))
$$
$$
{\sf id}_t : t \to t 
 \ \ \ \ \ \ 
 {\sf proj}^{l,k}_{t_i} \ : \ \times_{i \in l}. t_i \to t_k \ \ (k \in l)
$$
$$
 {\sf inj}^{l,k}_{t_i} \ : \ t_k \to +_{i \in l}. t_i \ \ (k \in l)
$$
 $$
{\sf tuple}^{l} \ \{ e_i : t' \to t_i \ | \ i \in l \} \ : \ t' \to \times_{i \in l}. t_i
$$
$$
{\sf case}^{l} \ \ \{ e_i : t_i \to t' \ | \ i \in l \} \ : \ +{i \in l}. t_i \to t'
 $$
under the usual axioms for indexed products and co-products:
$$
f \circ {\sf id} = f \ \ \ \ {\sf id} \circ f = f \ \ \ \ (f \circ g) \circ h = f \circ (g \circ h)
$$
$$
{\sf proj}^{l,k} \circ {\sf tuple}^{l} \ \{ e_i \ | \ i \in l \} \ = e_k 
$$
$$
{\sf case}^{l} \ \{ e_i \ | \ i \in l \} \circ {\sf inj}^{l,k} \ = e_k 
$$
$$
{\sf tuple}^{l} \ \{ {\sf proj}^{l,i} \circ f \ | \ i \in l \} \ = f 
\ \ \ \ \ \ 
{\sf case}^{l} \ \{ f \circ {\sf inj}^{l,i} \ | \ i \in l \} \ = f 
$$
We define $1 := \Pi_\emptyset. \emptyset$ and $0 := \Sigma_\emptyset. \emptyset$.  For every pair of distinguished labels ${\sf left}$ and ${\sf right}$, we may define binary products and co-products using $\{{\sf left}, {\sf right}\}$ as the indexing set.  The paper \cite{Gaster96apolymorphic} provides a sound and complete label inference system for the above grammar based on Haskell-like qualified types. 


==> gapgs.tex <==
\section{Generalized APGs}
\label{section.gapgs}



==> mappings.tex <==
% \section{Mapping to/from Other Data Models}
% \label{section.mmadt}

% In this section, we describe how various data models can be specified in terms of APGs plus data integrity constraints.
% Of course, it is not unexpected that APG can represent these other data models, as each model can also be defined as category of algebraic databases on a constrained schema in sense of~\cite{wadt}.  Currently, SPARQL is used for queries over APG schemas and data at Uber, with a translation of SPARQL into APG morphisms (see section~\ref{sec:ops}) forthcoming.

% % Other than Uber's Dragon (an APG extension which is described in \autoref{section.dragon}), these are all  ``model-ADTs''\footnote{\url{http://rredux.com/mm-adt/\#model-adts}} which have been proposed in connection with Apache TinkerPop version 4.   

% %{\bf Future Direction: More Model Morphisms.}  It is not unexpected that APG can represent these model-ADTs, as each model can also be defined as category of algebraic databases on a constrained schema in sense of~\cite{wadt}.
% %Note also that although an APG schema can define each model-ADT, APG gives no direct guidance about  any model-ADT-specific query languages one may wish to use to query a particular model-ADT, and similarly for updates.
% %It is possible to adapt a variety of existing query languages to APG; SPARQL is currently used for queries over APG schemas and data at Uber, while an exploration of other languages, such as Gremlin and Cypher, is left as a future direction.

% \subsection{Key-Value}
% \label{section.primary-keys}

% %It is straightforward to place data integrity constraints, such as primary key constraints, on APG data, and to use these constraints to implement other data models, such as the key-value model-ADT.
% Given an APG $G$, when $G(\pgsigma)(\pglabel{l}) = \pgtype{k} \times \pgtype{v}$ and ${\sf fst}(G(\pgupsilon)(\pgelement{e_1})) = {\sf fst}(G(\pgupsilon)(\pgelement{e_2})) \Rightarrow \pgelement{e_1} = \pgelement{e_2}$, we are justified in saying that $\pgtype{k}$ is a primary key for label $\pglabel{l}$, and we may treat the element as a key-value pair.
% For example, a suitable $\pgtype{k}$ is $\pgone + \pgone + \ldots + \pgone$ for some large but finite number of summands (or $\pgtypelit{Nat}$, the type of natural numbers); another suitable $\pgtype{k}$ is $\pglabel{l}$, which uses the element $\pgelement{e}$ as a primary key for itself, a similar technique to using all of a table's columns, as a primary key.  
% %There is no restriction on the languages that can be used to express constraints, but in practice we imagine some fragment of first-order logic to be a reasonable choice.

% \subsection{Relational}
% \label{sec:mmadtrelational}

% The relational model-ADT is represented in APG by requiring each APG label to map to a product type. 
% Our taxonomy (\autoref{section.taxonomy}) can be understood relationally in the same way.
% That is, each label of an APG has an associated algebraic data type $\pgtype{t}$.
% If we suppose that, for example $G(\pgsigma)(\pglabel{l}) = \pgtypelit{String} \times \pgtypelit{Nat}$ for a given label $\pglabel{l}$, then we can think of $\pglabel{l}$ as defining a table with two columns, the first holding strings and the second holding natural numbers, and we can store all elements $\pgelement{e}$ with $G(\pglambda)(\pgelement{e}) = \pglabel{l}$ in that table.
% In this way, many APG schemas can be completely understood and implemented using the relational model.
% However, our proposal goes beyond the traditional relational model by allowing domain values, i.e. the objects of relational tuples, to be structured as nested tuples and variants, as opposed to atomic in the sense of Codd. % (values only being allowed at base types).
% For example, consider values such as $((\pgvaluelit{37.78}, \pgvaluelit{-122.42}), inl(\pgvaluelit{1564061155}))$, which is a tuple of two objects, the first of which is itself a tuple -- a latitude/longitude pair -- and the second of which is a variant value which represents a choice of one alternative over another, such as a timestamp in seconds as opposed to a timestamp in milliseconds.
% %We may further extend this graphs-as-relations analogy, allowing relational notions of data integrity constraint such as primary keys (see \autoref{section.primary-keys}) to generalize to APGs.
% %At the limit of this analogy we arrive at {\it algebraic databases} \cite{wadt} and related formalisms.  

% \subsection{Triple Stores}
% \label{sec:mmadtrdf}

% %todo: Ryan and Josh: work on translating SPARQL queries 

% To represent an RDF graph as an APG requires a single label mapping to a type that is a three-fold product.  Alternatively, because RDF graphs are directed multi-graphs, we can represent them directly as categories with trivial composition relations, the so-called {\it free} categories (see \autoref{section.ct}).  In the reverse direction, representing an APG in a triple store is straightforward: let $C$ be a category and $F : C \to {\sf Set}$ a functor.  The category $\int F$, called the {\it category of elements} or {\it Grothendieck construction} for $F$, has for objects all pairs $(c, x)$ where $c \in {\sf Ob}(C)$ and $x \in F(c)$.  The morphisms from $(c, x)$ to $(c', x')$ are all the morphisms $f : c \to c'$ in $C$ such that $F(f)(x) = x'$.  Note that there is an obvious canonical functor $\partial : \int F \to C$.  Each category $\int F$ is generated by the graphs in \autoref{sec:vertices} (along with their implicit associated commutativity constraints, omitted in those diagrams), and can be stored (in e.g. RDF) using the usual graphs-as-triples encoding.  For example:

% \begin{centering}
% \vspace{-.2in}
% $$
% \xymatrix@=12pt{
% \LTO{\pgvalue{Alice}} & \LTO{\pgvalue{Bob}} & \LTO{\pgvalue{Chaz}} \ar[r]_{\pgtau} & \LTO{\pgtype{String}} & \LTO{\pgtype{User \times User}} & \LTO{\pgvalue{(u_1,u_2)}} \ar[l]^{\pgtau} & \LTO{\pgvalue{(u_1,u_3)}} \ar@/_1.5pc/[ll]_{\pgtau}  \\
% \LTO{\pgelement{u_1}} \ar[u]^{\pgupsilon} \ar@/_1pc/[rrr]_{\pglambda} & \LTO{\pgelement{u_2}} \ar[u]^{\pgupsilon} \ar@/^1pc/[rr]^{\pglambda} & \ar@/^1pc/[u]^{\pgupsilon}  \LTO{\pgelement{u_3}} \ar[r]^{\pglambda} & \LTO{\pglabel{User}}  \ar[u]^{\pgsigma} &
% \LTO{\pglabel{Trip}} \ar[u]^{\pgsigma} & \LTO{\pgelement{t_1}} \ar[u]^{\pgupsilon} \ar[l]_{\pglambda} & \LTO{\pgelement{t_2}}  \ar@/^1pc/[ll]^{\pglambda} \ar[u]^{\pgupsilon}
% }
% $$
% %\vspace{-.2in}
% \end{centering}
% \begin{footnotesize}
% \vspace{.15in}
% \hrulefill
% $$\hspace*{-.08in}
% \begin{tabular}{| c || c | c |}\bhline
% \multicolumn{3}{| c |}{$\pgE$lement}\\\bbhline 
% {\bf ID}&$\pglambda$&$\pgupsilon$\\\bbhline 
% $\pgelement{t_1}$& $\pglabel{\sf Trip}$ & $\pgvalue{(u_1,u_2)}$ \\\hline 
% $\pgelement{t_2}$& $\pglabel{\sf Trip}$ & $\pgvalue{(u_1,u_3)}$ \\\hline 
% $\pgelement{u_1}$& $\pglabel{\sf User}$ & $\pgvalue{\sf Alice}$ \\\hline 
% $\pgelement{u_2}$& $\pglabel{\sf User}$ & $\pgvalue{\sf Bob}$ \\\hline 
% $\pgelement{u_3}$& $\pglabel{\sf User}$ & $\pgvalue{\sf Chaz}$ \\\bhline 
% \end{tabular}
%  \ \ 
% \begin{tabular}{| c || c | }\bhline
% \multicolumn{2}{| c |}{$\pgV$alue}\\\bbhline 
% {\bf ID}&$\pgtau$\\\bbhline 
% $\pgvalue{\sf Alice}$ & \pgtype{String}  \\\hline 
% $\pgvalue{\sf Bob}$ & \pgtype{String}  \\\hline 
% $\pgvalue{\sf Chaz}$ & \pgtype{String}  \\\hline 
% $\pgvalue{(u_1,u_2)}$ & $\pgtype{\sf User\!\times\!User}$  \\\hline 
% $\pgvalue{(u_1,u_3)}$ & $\pgtype{\sf User\!\times\!User}$ \\\bhline 
% \end{tabular}
% $$
% $$
% \begin{tabular}{| c || c | }\bhline
% \multicolumn{2}{| c |}{$\pgL$abel}\\\bbhline 
% {\bf ID}&$\pgsigma$\\\bbhline 
% $\pglabel{\sf User}$& $\pgtype{\sf String}$ \\\hline 
% $\pglabel{\sf Trip}$& $\pgtype{\sf User\!\times\!User}$   \\\bhline 
% \end{tabular}
% \ \
% \begin{tabular}{| c |}\bhline
% \multicolumn{1}{| c |}{$\pgT$ype}\\\bbhline 
% {\bf ID}\\\bbhline 
% \pgtype{String} \\\hline 
% $\pgtype{\sf User\!\times\!User}$  \\\bhline 
% \end{tabular}
% $$
% \end{footnotesize}

% Slightly more idiomatic mappings, leveraging OWL, are used for the translation of APG schemas and data to RDF/OWF at Uber; an OWL-based mapping is used for exporting schemas to ontology editors such as Prot\'eg\'e and Gra.fo, while a more faithful and complete mapping based on SHACL is used for supporting SPARQL queries over schemas and data; the APG schemas of Dragon (see below) can be seen as a proper subset of SHACL.

% \subsection{Nested Data}

% There are at least two strategies for representing JSON and other nested datasets such as XML.  The first is to transform the nested relational datasets into flat relational datasets using the traditional technique of shredding of nested data into parent/child foreign keys ~\cite{Bussche1999SimulationOT}.  The second is to add collection types such as Dragon's, and exploit the tree-structured nature of algebraic data types~\cite{grust}.
% This is what is done for YAML and JSON in Dragon.
% For example, a type such as ${\sf List} \ (\pgtype{{\sf Int}} \times ({\sf List} \ \pgtype{{\sf String}})))$ contains nested lists.
% %An example of this shredding process is shown in \autoref{fig:shredding}.
 
% %\begin{figure}[h]
% %\begin{footnotesize}
% % \begin{sf}
% % $$
% % \begin{tabular}{c|c|c}
% % name     & age & kids  \\ \hline
% % bill & 30 & 
% % \begin{tabular}{c|c|c}
% % gender    & name  & friends \\ \hline
% %   F   & sue & \begin{tabular}{c} name \\ \hline kid1 \\ kid3 %\end{tabular} \\
% %   F & alice & \begin{tabular}{c} name \\ \hline kid1 \\ kid2 %\end{tabular} \\
% %   M & joe & \begin{tabular}{c} name \\ \hline kid3 \end{tabular} \\
% % \end{tabular}
% % \\ 
% % bob & 40 & 
% %  \begin{tabular}{c|c|c}
% % gender  & name & friends \\ \hline
% %   F   & kim & \begin{tabular}{c} name \\ \hline kid1 \\ kid2 %\\ kid3 \end{tabular} \\
% %   M & chuck & \begin{tabular}{c} name \\ \hline %\end{tabular} \\
% % \end{tabular}
% % \end{tabular}$$
% % \\ 
% % $$
% % \downarrow 
% %$$ 
% %\\ 
% %$$
%  %\begin{tabular}{c|c}
%  %name     & ID  \\ \hline
%  %kid1     & 6   \\
%  %kid1     & 4   \\
%  %kid1     & 5   \\
%  %kid2     & 5   \\
%  %kid2     & 4   \\
%  %kid3     & 6   \\
%  %kid3     & 3   \\
%  %kid3     & 5   \\
%  %\end{tabular}
%  %\ \ 
%  %\begin{tabular}{c|c|c|c}
%  %gender & name     & ID & friends \\ \hline 
%  %F     & kim & 1 & 5   \\
%  % F     & alice & 0 & 4   \\
%  %  F     & sue & 0 & 6   \\
%  %   M     & chuck & 1 & 2   \\
%  %    M     & joe & 0 & 3   \\
%  %    \\
%   %  
%   %  name     & age & kids  \\ \hline
% % bill     & 30 & 0   \\
% % bob     & 40 & 1   \\     
% % \end{tabular}
% % $$
% %% \end{sf}
% %\end{footnotesize}
% %\caption{Nested-relational Shredding}
% %\label{fig:shredding}
% %\end{figure}
 

==> taxonomy.tex <==
\section{Taxonomy of graph elements}
\label{section.taxonomy}

%Todo: Josh: Use logic to define the formulae that characterize the taxonomy classes.  For example, label $\pglabel{l}$ is a vertex when the following formula holds:
%$$\pgsigma({\sf c}_{\pglabel{l}}) = {\sf c}_{\pgone}$$


In this section, we develop a taxonomy for classifying property graph elements according to their associated labels and schemas.
The principal use of this taxonomy is in interfacing non-graph data sources with property graph frameworks, primarily Apache TinkerPop.

By analogy with the mathematical notion of a \textit{graph}, property graphs are usually described in terms of \textit{vertices} and \textit{edges},\footnote{Or \textit{nodes} and \textit{relationships}, in addition to similar terms.} collectively termed \textit{elements}, in addition to \textit{properties}.\footnote{In this paper, properties are treated as elements, as well. This approach is consistent with the usual notion of properties as key/value pairs attached to vertices or edges, while it also allows for meta-properties.}
% For example, a \pglabellit{name} property might connect a \pglabellit{User}-vertex to a \pgtypelit{String} value.  
% Properties themselves are frequently subdivided according to the class of element they attach to; thus, we have \textit{vertex properties}, \textit{edge properties}, and even \textit{meta-properties}.
We now provide concrete definitions for these and other concepts in terms of the APG data model defined above.
% Further extending this taxonomy and formalizing its use for various data-related tasks is an important direction for future work.  
{\it Note that in this section we are always working with respect to a particular APG $G$, which for the sake of brevity, we will not re-introduce in each subsection}.

\subsection{Vertices}
\label{sec:vertices}
A {\it vertex label} is a label $\pglabel{l}$  such that $G(\pgsigma)(\pglabel{l}) = \pgone$, i.e. a vertex is an element with ``no data''.
An $\pglabel{l}$-{\it vertex} is an element $\pgelement{e}$ such that $G(\pglambda)(\pgelement{e}) = \pglabel{l}$ where $\pglabel{l}$ is a vertex label.  Using our four-sorted logic, the set of vertex labels is definable using the formula ${\sf vertexlabel}(l {:} \pgL) := \pgsigma(\pglabel{l}) = \pgtype{1}$.
The set of vertices is definable using the formula ${\sf vertex}(e {:} \pgE) :={\sf vertexlabel}(\pglambda(e))$.  
Consider a graph containing a \pglabellit{User}-vertex $\pgelement{u_1}$ and a \pglabellit{Trip}-vertex $\pgelement{t_1}$ as in the examples above:

\begin{footnotesize}
\begin{align*}
& G(\pgL) := \{ \pglabellit{User}, \pglabellit{Trip} \}
\ \ \ \ 
G(\pgE) := \{ \pgelement{u_1}, \pgelement{t_1} \}
\ \ \ \ 
G(\pgupsilon)(\pgelement{u_1}) := G(\pgupsilon)(\pgelement{t_1}) := \pgunit \\
& G(\pgsigma)(\pglabellit{User}) := G(\pgsigma)(\pglabellit{Trip}) := \pgone
\ \ \ \ 
G(\pglambda)(\pgelement{u_1}) := \pglabellit{User}
\ \ \ \
G(\pglambda)(\pgelement{t_1}) := \pglabellit{Trip}
\end{align*}
\end{footnotesize}
We can display this graph visually:
\begin{footnotesize}
$$
\xymatrix@R-1.5pc{
  & \pgelement{u_1} \ar@/_1pc/[ld]_{\pgupsilon} \ar[r]^{\pglambda} & \pglabellit{User} \ar@/^1pc/[rd]^{\pgsigma} & \\
\pgunit \ar[rrr]^{\pgtau} &   &   & \pgone \\
  & \pgelement{t_1} \ar@/^1pc/[lu]^{\pgupsilon} \ar[r]_{\pglambda} & \pglabellit{Trip} \ar@/_1pc/[ru]_{\pgsigma} & \\
}
$$
\end{footnotesize}
A designated label, such as the empty string $\pglabel{\epsilon}$, may be used as the label of otherwise ``unlabeled'' vertices.
There is no difference between the value of a labeled and an unlabeled vertex; in both cases, the value is $\pgunit$.

\subsection{Edges}
\label{section.edges}

An ordinary, binary {\it edge label} is a label $\pglabel{l}$ such that $G(\pgsigma)(\pglabel{l}) = \pglabel{l_1} \times \pglabel{l_2}$ for vertex labels $\pglabel{l_1}, \pglabel{l_2}$.
An $\pglabel{l}$-{\it edge} is an element $\pgelement{e}$ such that $G(\pglambda)(\pgelement{e}) = \pglabel{l}$ where $\pglabel{l}$ is an edge label.
Using our four-sorted logic, the set of binary edge labels is definable using the formula
$$
 {\sf edgelabel}(\pglabel{l} {:} \pgL) := \exists \pglabel{l'}{:} \pgL, \ \exists \pglabel{l''} {:} \pgL, \ \pgsigma(\pglabel{l}) = \pglabel{l'} \times \pglabel{l''}  
 \wedge {\sf vertexlabel}(\pglabel{l'}) \wedge {\sf vertexlabel}(\pglabel{l''})
$$
and the set of binary edges can be defined as ${\sf edge}(\pgelement{e} {:} \pgE) :={\sf edgelabel}(\pglambda(\pgelement{e})).$

For example, consider a graph containing a \pglabellit{driver}-edge $\pgelement{d_1}$ and a \pglabellit{rider}-edge $\pgelement{r_1}$, which connect $\pglabellit{Trip}$-vertex $\pgelement{t_1}$ to $\pglabellit{User}$-vertices $\pgelement{u_1}$ and $\pgelement{u_2}$, respectively:
\begin{footnotesize}
\begin{align*}
& G(\pgL) := \{ \pglabellit{User}, \pglabellit{Trip}, \pglabellit{driver}, \pglabellit{rider} \} \\
& G(\pgsigma)(\pglabellit{User}) := G(\pgsigma)(\pglabellit{Trip}) := \pgone \\
& G(\pgsigma)(\pglabellit{driver}) := G(\pgsigma)(\pglabellit{rider}) := \pglabellit{Trip} \times \pglabellit{User} \\
& G(\pgE) := \{ \pgelement{t_1}, \pgelement{u_1}, \pgelement{u_2}, \pgelement{d_1}, \pgelement{r_1} \} \\
& G(\pglambda)(\pgelement{u_1}) := G(\pglambda)(\pgelement{u_2}) := \pglabellit{User}
\ \ \ \
G(\pglambda)(\pgelement{t_1}) := \pglabellit{Trip} \\
& G(\pglambda)(\pgelement{d_1}) := \pglabellit{driver}
\ \ \ \
G(\pglambda)(\pgelement{r_1}) := \pglabellit{rider} \\
& G(\pgupsilon)(\pgelement{u_1}) := G(\pgupsilon)(\pgelement{u_2}) := G(\pgupsilon)(\pgelement{t_1}) := \pgunit \\
& G(\pgupsilon)(\pgelement{d_1}) := ({\pgelement{t_1}}, {\pgelement{u_1}})
\ \ \ \
G(\pgupsilon)(\pgelement{r_1}) := ({\pgelement{t_1}}, {\pgelement{u_2}})
\end{align*}
\end{footnotesize}
We have used the term ``ordinary'' because there are many other kinds of elements which do not satisfy the definition above, and yet may be considered ``edges'' in certain contexts.
For example, suppose we have a label $\pglabellit{owner}$ where $G(\pgsigma)(\pglabellit{owner}) = \pglabellit{Vehicle} \times (\pglabellit{User} + \pglabellit{Organization})$, and $\pglabellit{Vehicle}$, $\pglabellit{User}$, and $\pglabellit{Organization}$ are all vertex labels.
This useful construction allows either a user or an organization to be provided as the owner of a vehicle.

Certain property graph data models even allow higher-order edges, occasionally called \textit{meta-edges}.
Accommodating such elements in APG is just a matter of modifying the above reference to ``vertex labels'' to labels of an appropriate kind.
For example, we might define ``edge-vertex edges'' in terms of edge labels $\pglabel{l}$ with $G(\pgsigma)(\pglabel{l}) = \pglabel{l_1} \times \pglabel{l_2}$, where $\pglabel{l_1}$ is an ordinary edge label and $\pglabel{l_2}$ is a vertex label.
There is an endless variety of such patterns.
Similarly, we can generalize to $n$-ary edges (\autoref{section.hyperelements}), or to indexed edges~\cite{seely}.

%\subsubsection{Vertex Property}
%A vertex property connects a vertex to a primitive value.
%For example, \texttt{name} connects a \texttt{Person} to a \texttt{String}.  

\subsection{Properties}
\label{section.properties}

An ordinary {\it vertex property label}\footnote{Although we use the term ``property label'' in this paper for consistency, the term ``property key'' is more conventional.} is a label $\pglabel{l}$ such that $G(\pgsigma)(\pglabel{l}) = \pglabel{l'} \times \pgtype{p}$ for vertex label $\pglabel{l'}$ and \textit{primitive type} $\pgtype{p} \in \pgprimitives$.
An $\pglabel{l}$-{\it vertex  property} is an element $\pgelement{e}$ such that $G(\pglambda)(\pgelement{e}) = \pglabel{l}$ where $\pglabel{l}$ is a vertex label.
Using our four-sorted logic, let us define the predicate ${\sf primitive}(\pgtype{t} {:} \pgT) := \pgtype{t} = \pgtype{p_1} \vee \pgtype{t} = \pgtype{p_2} \vee \ldots$, where $\pgtype{p_1}$, $\pgtype{p_2}$, $\ldots$, are the primitive types of our APG.
Then the set of vertex property labels can be defined using the formula 
$$
{\sf vplabel}(\pglabel{l} {:} \pgL) := \exists \pglabel{l'} {:} \pgL, \ \exists \pgtype{t} {:} \pgT, \  \pgsigma(\pglabel{l}) = \pglabel{l'} \times \pgtype{t} \ \ \wedge {\sf vertexlabel}(\pglabel{l'}) \wedge {\sf primitive}(\pgtype{t}).
$$
%The set of binary edges can be defined as ${\sf edge}(y) :={\sf edgelabel}(\lambda(y))$ where $y$ is a variable of sort $\pgE$.  

For example, let $\pgprimitives$ include primitive type \pgtypelit{String}, and consider a graph containing a single \pglabellit{User}-vertex $\pgelement{u_1}$ with two  \pglabellit{name}-properties $\pgelement{n_1}, \pgelement{n_2}$:
\begin{footnotesize}
\begin{align*}
& G(\pgL) := \{ \pglabellit{User}, \pglabellit{name} \} \\
& G(\pgsigma)(\pglabellit{User}) := \pgone
 \ \ \ \
 G(\pgsigma)(\pglabellit{name}) := \pglabellit{User} \times \pgtypelit{String} \\
& G(\pgE) := \{ \pgelement{u_1}, \pgelement{n_1}, \pgelement{n_2} \} \\
& G(\pglambda)(\pgelement{u_1}) := \pglabellit{User}
\ \ \ \ 
G(\pglambda)(\pgelement{n_1}) := G(\pglambda)(\pgelement{n_2}) := \pglabellit{name} \\
& G(\pgupsilon)(\pgelement{u_1}) := \pgunit
 \ \ \ \ 
G(\pgupsilon)(\pgelement{n_1}) := ({\pgelement{u_1}}, \pgvaluelit{Arthur Dent}) \\
& G(\pgupsilon)(\pgelement{n_2}) := ({\pgelement{u_1}}, \pgvaluelit{Arthur P. Dent})
\end{align*}
\end{footnotesize}
So called \textit{multi-properties}, i.e. properties with the same label outgoing from the same element, are supported by default in APGs.
In the example above, the $\pglabellit{User}$ vertex $\pgelement{u_1}$ has two distinct $\pglabellit{name}$ properties, which happen to have different values.
In order to \textit{disallow} multi-properties, we must add a uniqueness constraint:
$$
%\forall \pgelement{e}, \pgelement{p_1}, \pgelement{p_2} \in G(\pgE) :
%\forall \pgtype{t} \in G(\pgT) :\quad
(G(\pglambda)(\pgelement{e}) = G(\pglambda)(\pgelement{e'}) = \pglabel{l}) \Rightarrow
(G(\pgupsilon)(\pgelement{e}) = G(\pgupsilon)(\pgelement{e'}) \Rightarrow \pgelement{e} = \pgelement{e'})
%G(\pgupsilon)(\pgelement{p_1}) := G(\pgupsilon)(\pgelement{p_2}) := (\pgelement{e}, \pgtype{t}) 
%\Rightarrow \pgelement{p_1} = \pgelement{p_2}
$$
where $\pglabel{l}$ is a property label as defined above.  %Syntactically:
%$$
%\forall e{:}\pgE , e'{:}\pgE, \ {\sf vplabel}(\pglambda(e)) \Rightarrow \pglambda(e) = \pglambda(e') \Rightarrow \pgupsilon(e) = \pgupsilon(e') \Rightarrow e = e'.
%$$

Apart from vertex properties, most property graph implementations also support \textit{edge properties}.
An ordinary {\it edge property label} is a label $\pglabel{l}$ such that $G(\pgsigma)(\pglabel{l}) = \pglabel{l'} \times \pgtype{p}$ for edge label $\pglabel{l'}$ and primitive type $\pgtype{p} \in \pgprimitives$.
For example, we may attach a $\pglabellit{driverStatus}$ property to the $\pglabellit{driver}$ edge defined in \autoref{section.edges}, where
$
G(\pgsigma)(\pglabellit{driverStatus}) = \pglabellit{driver} \times \pgtypelit{String}
$.

We have used the term ``ordinary'' above to distinguish typical vertex and edge properties from so-called \textit{meta-properties}, i.e. properties of properties.
Rather than saying ``vertex property property'' we say ``vertex meta-property''.
By analogy, one can speak of ``edge meta-properties'', although these are uncommon in practice.
For example, we may add a $\pgtypelit{Double}$-valued $\pglabellit{confidence}$ meta-property to the $\pglabellit{name}$ property in the example above.

One can easily generalize the value type of ``ordinary'' properties from primitive types to arbitrary types that do not contain labels, such as $\pgtypelit{Integer} + \pgtypelit{String}$, or for  more expressiveness, we may allow labels, keeping properties distinct from edges by requiring only that we can recursively ``dereference'' all labels to obtain a primitive type, or a type expression in which all leaf nodes are primitive types.
For example, if $G(\pgsigma)(\pglabellit{driverStatus}) = \pglabellit{driver} \times \pglabellit{Status}$ and $G(\pgsigma)(\pglabellit{Status}) = \pgtypelit{String}$, then $\pglabellit{driverStatus}$ is still a generalized property label.
The $\pglabellit{Status}$ label is called an {\it alias}; see below.

% \subsection{Aliases}
% We use the term ``element'' more broadly in this paper than we do in Apache TinkerPop. 
% Vertices and edges are elements, but so are properties, as well as all other types to which we have given a label.
% Whereas the value of an edge or property contains two other values, and the value of a vertex contains no values, the elements we call \textit{aliases} contain a single value.
% Specifically, a {\it data type alias} is a label $\pglabel{l}$ such that $G(\pgsigma)(\pglabel{l})$ is a primitive type $\pgtype{p} \in {\sf P}$.
% In other words, we can define
% $${\sf dtaliaslabel}(\pglabel{l} : \pgL) := {\sf primitive}(\pgsigma(\pglabel{l})).
% $$
% More generally, we may consider any type not containing labels by using an inductively defined predicate {\sf dtaliaslabel'}:
% \begin{align*}
% &{\sf dtaliaslabel'}(\pgzero) := {\sf true} \ \ \
% {\sf dtaliaslabel'}(\pgone) := {\sf true} \\
% & {\sf dtaliaslabel'}({\sf Prim} \ \pgtype{p}) := {\sf true} \ \ \ 
% {\sf dtaliaslabel'}({\sf Lbl} \ \pglabel{l}) := {\sf false} \\ 
% & {\sf dtaliaslabel'}(\pgtype{t_1} + \pgtype{t_2}) := {\sf dtaliaslabel'}(\pgtype{t_1}) \wedge {\sf dtaliaslabel'}(\pgtype{t_2})  \\
% & {\sf dtaliaslabel'}(\pgtype{t_1}  \wedge \pgtype{t_2}) := {\sf dtaliaslabel'}(\pgtype{t_1})\wedge {\sf dtaliaslabel'}(\pgtype{t_2}) 
% \end{align*}
% or more generally still, we may require only that $\pglabel{l}$ ``dereferences'' to a type that does not contain labels; see  \autoref{section.properties} above, which we formalize inductively as {\sf dtaliaslabel''}:
% \begin{align*}
% &{\sf dtaliaslabel''}(\pgzero) := {\sf true} \ \ \
% {\sf dtaliaslabel''}(\pgone) := {\sf true} \\
% & {\sf dtaliaslabel''}({\sf Prim} \ \pgtype{p}) := {\sf true} \ \ \ 
% {\sf dtaliaslabel''}({\sf Lbl} \ \pglabel{l}) := {\sf dtaliaslabel'}(\pgsigma(\pglabel{l})) \\ 
% & {\sf dtaliaslabel'}(\pgtype{t_1} + \pgtype{t_2}) := {\sf dtaliaslabel''}(\pgtype{t_1}) \wedge {\sf dtaliaslabel''}(\pgtype{t_2})  \\
% & {\sf dtaliaslabel''}(\pgtype{t_1}  \wedge \pgtype{t_2}) := {\sf dtaliaslabel''}(\pgtype{t_1})\wedge {\sf dtaliaslabel''}(\pgtype{t_2}) 
% \end{align*}
% For example, consider a graph and schema in which \pglabellit{DegreesLatitude} and \pglabellit{DegreesLongitude} are both aliases for a primitive \pgtypelit{Double} type, the values of which are numbers such as $\pgvaluelit{37.78}$ and $\pgvaluelit{-122.42}$:
% %label in $G(\pgL)$ for simple values, such as strings and numbers, are distinct from primitive types in $B$.
% \begin{footnotesize}
% \begin{align*}
% & G(\pgL) := \{ \pglabellit{DegreesLatitude}, \texttt{ \pglabel{DegreesLongitude}} \} \\
% & G(\pgsigma)(\pglabellit{DegreesLatitude}) := G(\pgsigma)(\pglabellit{DegreesLongitude}) := \pgtypelit{Double} \\
% & G(\pgE) := \{ \pgelement{d_1}, \pgelement{d_2} \} \\
% & G(\pglambda)(\pgelement{d_1}) := \pglabellit{DegreesLatitude}
% \ \ \ \ 
% G(\pglambda)(\pgelement{d_2}) := \pglabellit{DegreesLongitude} \\
% & G(\pgupsilon)(\pgelement{d_1}) := \pgvaluelit{37.78}
% \ \ \ \ 
% G(\pgupsilon)(\pgelement{d_2}) := \pgvaluelit{-122.42}
% \end{align*}
% \end{footnotesize}
% % We may generalize this definition by allowing $G(\pgsigma)(\pglabel{l})$ to be any type, such as $\pgtypelit{String} \times \pgtypelit{String}$, thereby allowing for arbitrary data.
% Another useful kind of alias is a {\it vertex tag}.
% This term is not commonplace in property graph APIs, but tags frequently crop up in enterprise settings, where they may serve as a kind of unary ``edge'' which is simpler than either a (binary) edge or a property.
% Specifically, a {\it vertex tag label} is a label $\pglabel{l}$ for which $G(\pgsigma)(\pglabel{l}) = \pglabel{l'}$, where $\pglabel{l'}$ is a vertex label.
% {\it Edge tag labels}, {\it property tag labels}, and so on can be defined in an analogous way.
% A {\it vertex tag}, {\it edge tag}, etc. is an element $\pgelement{e}$ such that $G(\pglambda)(\pgelement{e}) = \pglabel{l}$, where $\pglabel{l}$ is a tag label of the appropriate kind.
% For example, consider tag labels $\pglabellit{Completed}$ and $\pglabellit{Updated}$, which are to be applied to $\pglabellit{Trip}$ vertices:
% \begin{footnotesize}
% \begin{align*}
% & G(\pgL) := \{ \pglabellit{Trip}, \pglabellit{Completed}, \pglabellit{Updated} \} \\
% & G(\pgsigma)(\pglabellit{Trip}) := \pgone
% \ \ \ 
% G(\pgsigma)(\pglabellit{Completed}) := G(\pgsigma)(\pglabellit{Updated}) := \pglabellit{Trip} \\
% & G(\pgE) := \{ \pgelement{t_1}, \pgelement{t_2}, \pgelement{c_1}, \pgelement{c_2}, \pgelement{u_1} \} \\
% & G(\pglambda)(\pgelement{t_1}) := G(\pglambda)(\pgelement{t_2}) := \pglabellit{Trip} \\
% & G(\pglambda)(\pgelement{c_1}) := G(\pglambda)(\pgelement{c_2}) := \pglabellit{Completed}
% \ \ \ \ 
% G(\pglambda)(\pgelement{u_1}) := \pglabellit{Updated} \\
% & G(\pgupsilon)(\pgelement{t_1}) := \pgunit
% \ \ \ \
% G(\pgupsilon)(\pgelement{c_1}) := {\pgelement{t_1}}
% \ \ \ \
% G(\pgupsilon)(\pgelement{c_2}) := {\pgelement{t_2}}
% \ \ \ \
% G(\pgupsilon)(\pgelement{u_1}) := {\pgelement{t_2}}
% \end{align*}
% \end{footnotesize}
% This graph expresses that trips $\pgelement{t_1}$ and $\pgelement{t_2}$ are both $\pglabellit{Completed}$, whereas $\pgelement{t_2}$ is also $\pglabellit{Updated}$.
% As the tags are themselves elements, an application could extend this schema by adding property labels that qualify the tagging relationships, such as $\pglabellit{asOfTime}$ or $\pglabellit{comments}$.

\subsection{Hyperelements}
\label{section.hyperelements}

Although the reader might expect {\it hyperelements}, i.e. generalized relationships, to be complicated, they are in fact the simplest kind of label in this taxonomy: literally every possible label is a hyperelement label.
Nonetheless, it is sometimes useful to describe as ``hyperedges'' or ``hyperelements'' those labels that do not belong to any more constrained class in the taxonomy.
In the following graph, for example, we directly translate the example from \autoref{figure.rdf-graph} by treating a $\pglabellit{Trip}$ element not as a vertex, nor as a binary edge, but as a hyperelement; every $\pglabellit{Trip}$ connects two $\pglabellit{User}$ vertices and up to two $\pglabellit{PlaceEvent}$ elements.
We will also add a timestamp field:

% The primary key of the $\pglabellit{Trip}$, called ${\sf id}$ in the Thrift IDL example, is implicit.
% We will illustrate the schema using the RDF example graph from \autoref{figure.rdf-graph}, also adding a timestamp field:
\begin{footnotesize}
\begin{align*}
& G(\pgL) := \{ \pglabellit{User}, \pglabellit{Trip}, \pglabellit{PlaceEvent}, \pglabellit{Place}, \pglabellit{UnixTimeSeconds} \} \\
& G(\pgsigma)(\pglabellit{User}) := G(\pgsigma)(\pglabellit{Place}) := \pgone \\
& G(\pgsigma)(\pglabellit{PlaceEvent}) := \pglabellit{Place} \times \pglabellit{UnixTimeSeconds} \\
& G(\pgsigma)(\pglabellit{UnixTimeSeconds}) := \pgtypelit{Integer} \\
& G(\pgsigma)(\pglabellit{Trip}) := \pglabellit{User} \times \pglabellit{User} \times (\pgone + \pglabellit{PlaceEvent}) \times (\pgone + \pglabellit{PlaceEvent}) \\
& G(\pgE) := \{ \pgelement{u_1}, \pgelement{u_2}, \pgelement{u_3}, \pgelement{t_1}, \pgelement{t_2},   \pgelement{e_1}, \pgelement{e_2}, \pgelement{e_3}, \pgelement{e_4}, \pgelement{p_1}, \pgelement{p_2}, \pgelement{p_3}, \pgelement{s_1}, \pgelement{s_2}, \pgelement{s_3}, \pgelement{s_4} \} \\
& G(\pglambda)(\pgelement{u_1}) := G(\pglambda)(\pgelement{u_2}) := G(\pglambda)(\pgelement{u_3}) := \pglabellit{User}
\ \ \ \
G(\pglambda)(\pgelement{t_1}) := G(\pglambda)(\pgelement{t_2}) := \pglabellit{Trip} \\
& G(\pglambda)(\pgelement{p_1}) := G(\pglambda)(\pgelement{p_2}) := G(\pglambda)(\pgelement{p_3}) := \pglabellit{Place} \\
& G(\pglambda)(\pgelement{e_1}) := G(\pglambda)(\pgelement{e_2}) := G(\pglambda)(\pgelement{e_3}) :=
G(\pglambda)(\pgelement{e_4}) := \pglabellit{PlaceEvent} \\
& G(\pglambda)(\pgelement{s_1}) := G(\pglambda)(\pgelement{s_2}) := G(\pglambda)(\pgelement{s_3}) := G(\pglambda)(\pgelement{s_4}) := \pglabellit{UnixTimeSeconds} \\
& G(\pgupsilon)(\pgelement{u_1}) := G(\pgupsilon)(\pgelement{u_2}) := G(\pgupsilon)(\pgelement{u_3}) := G(\pgupsilon)(\pgelement{p_1}) := G(\pgupsilon)(\pgelement{p_2}) := G(\pgupsilon)(\pgelement{p_3}) := \ \pgunit \\
% note: to save space, using inl and inr instead of inl_{(1+PlaceEvent)}
& G(\pgupsilon)(\pgelement{t_1}) := ({\pgelement{u_1}}, {\pgelement{u_2}}, {\sf inr}({\pgelement{e_1}}), {\sf inr}({\pgelement{e_2}})) 
\ \ \ \
G(\pgupsilon)(\pgelement{t_2}) := ({\pgelement{u_1}}, {\pgelement{u_3}}, {\sf inr}({\pgelement{e_3}}), {\sf inl}(\pgunit)) \\
& G(\pgupsilon)(\pgelement{e_1}) := ({\pgelement{p_1}}, {\pgelement{s_1}})
\ \ \ \
G(\pgupsilon)(\pgelement{e_2}) := ({\pgelement{p_2}}, {\pgelement{s_2}}) \\
& G(\pgupsilon)(\pgelement{e_3}) := ({\pgelement{p_2}}, {\pgelement{s_3}})
\ \ \ \
G(\pgupsilon)(\pgelement{e_4}) := ({\pgelement{p_3}}, {\pgelement{s_4}}) \\
& G(\pgupsilon)(\pgelement{s_1}) := \pgvaluelit{1602203601}
\ \ \ \
G(\pgupsilon)(\pgelement{s_2}) := \pgvaluelit{1602203948} \\
& G(\pgupsilon)(\pgelement{s_3}) := \pgvaluelit{1602204122}
\ \ \ \
G(\pgupsilon)(\pgelement{s_4}) := \pgvaluelit{1602205255}
\end{align*}
\end{footnotesize}
Note that the $\pglabellit{User}$-valued fields are ``required'' in $\pglabellit{Trip}$, whereas $\pglabellit{PlaceEvent}$ fields are ``optional''; per the example, trip $\pgelement{t_2}$ has a \texttt{pickup} event, but no \texttt{dropoff} event.
This optionality is encapsulated in the type $\pgone + \pglabellit{PlaceEvent}$; values with this type are either a trivial value ${\sf inl}(\pgunit)$, i.e. the unit value $\pgunit$ ``on the left'', or a value ${\sf inr}({\sf Elmt} \ \pgelement{e})$ ``on the right'', where $\pgelement{e}$ is a $\pglabellit{PlaceEvent}$ element.
Note also that even though $\pglabellit{PlaceEvent}$ elements have the shape of (generalized) vertex properties, we choose not to think of them as such because $\pglabellit{PlaceEvent}$ does not have the intuitive semantics of a property label.

The above is a realistic, although simplified, enterprise schema; no clear distinction has been made between vertices, edges, and properties, as in this case, such a distinction is not useful.
Nonetheless, we can treat the graph as a ``property graph'' insofar as we can readily perform path-finding operations, compute connected components, and so on, in addition to many other operations we typically perform on more conventional graph datasets.

% \subsection{Paths}
% \label{section.paths}

% Let $(\pgelement{v_0},\ldots \pgelement{v_n})$ be a list of vertices and $(\pgelement{e_1}, \ldots \pgelement{e_n})$ be a list of binary edges such that $G(\pgupsilon)(e_i)=(\pgelement{v_{i-1}},\pgelement{v_i})$ for each $i=1,\ldots,n$.  Then we say that this list of edges is a \textit{path} from $\pgelement{v_0}$ to $\pgelement{v_n}$ .

% Our four-sorted logic can say that a certain path from $\pgelement{v_0}$ to $\pgelement{v_n}$ is the shortest path from $\pgelement{v_0}$ to $\pgelement{v_n}$.  In the case $n=2$, this amounts to the nonexistence of any paths of length $0$ or $1$, or any \textit{other} paths of length $2$:
% \begin{align*}
% & \neg (\pgelement{v_0}=\pgelement{v_2}) \wedge \forall \pgelement{f_1} {:} \pgE \ [ \neg(\pgupsilon(\pgelement{f_1})=(\pgelement{v_0},\pgelement{v_2})) \\
% & \wedge \forall \pgelement{f_2}, \pgelement{v} {:} \pgE \
% (\pgupsilon(\pgelement{f_1})=(\pgelement{v_0},\pgelement{v}) \wedge \pgupsilon(\pgelement{f_2})=(\pgelement{v},\pgelement{v_2})) \Rightarrow (\pgelement{f_1}=\pgelement{e_1} \wedge \pgelement{f_2}=\pgelement{e_2}) ]
% \end{align*}

% In fact, every first-order sentence over a graph $(V,E, s,t:V\rightarrow E)$ can be lifted to a sentence in our four-sorted logic over an APG that encodes $(V,E)$, by recursively making the following transformations, where $\mathcal{S}$ is an arbitrary sentence and $\mathcal{S}[a/x]$ denotes substitution of $a$ for some free variable $x$ in $\mathcal{S}$:

% \begin{align*}
%     \forall v {:} V ,\ \mathcal{S}[v/x] & \ \mapsto\ \forall \pgelement{v} {:} \pgE, \ {\sf vertex}(\pgelement{v}) \Rightarrow \mathcal{S}[\pgelement{v}/x] \\
%     \exists v {:} V ,\ \mathcal{S}[v/x] & \ \mapsto\ \exists \pgelement{v} {:} \pgE, \ {\sf vertex}(\pgelement{v}) \wedge \mathcal{S}[\pgelement{v}/x] \\
%     \forall e {:} E ,\ \mathcal{S}[e/x] & \ \mapsto\ \forall \pgelement{e} {:} \pgE, \ {\sf edge}(\pgelement{e}) \Rightarrow \mathcal{S}[\pgelement{e}/x] \\
%     \exists e {:} E ,\ \mathcal{S}[e/x] & \ \mapsto\ \exists \pgelement{e} {:} \pgE, \ {\sf edge}(\pgelement{e}) \wedge \mathcal{S}[\pgelement{e}/x] \\
%     \mathcal{S}[s(e)/x] & \ \mapsto\ \exists \pgelement{v_1},\pgelement{v_2} {:} \pgE, \ \pgupsilon(\pgelement{e})=(\pgelement{v_1},\pgelement{v_2}) \wedge \mathcal{S}[\pgelement{v_1}/x] \\
%     \mathcal{S}[t(e)/x] & \ \mapsto\ \exists \pgelement{v_1},\pgelement{v_2} {:} \pgE, \ \pgupsilon(\pgelement{e})=(\pgelement{v_1},\pgelement{v_2}) \wedge \mathcal{S}[\pgelement{v_2}/x] \\
% \end{align*}
